Efficient Formal Safety Analysis of Neural Networks

Neural networks are increasingly deployed in real-world safety-critical domains such as autonomous driving, aircraft collision avoidance, and malware detection. However, these networks have been shown to often mispredict on inputs with minor adversarial or even accidental perturbations. Consequences of such errors can be disastrous and even potentially fatal as shown by the recent Tesla autopilot crash. Thus, there is an urgent need for formal analysis systems that can rigorously check neural networks for violations of different safety properties such as robustness against adversarial perturbations within a certain $L$-norm of a given image. An effective safety analysis system for a neural network must be able to either ensure that a safety property is satisfied by the network or find a counterexample, i.e., an input for which the network will violate the property. Unfortunately, most existing techniques for performing such analysis struggle to scale beyond very small networks and the ones that can scale to larger networks suffer from high false positives and cannot produce concrete counterexamples in case of a property violation. In this paper, we present a new efficient approach for rigorously checking different safety properties of neural networks that significantly outperforms existing approaches by multiple orders of magnitude. Our approach can check different safety properties and find concrete counterexamples for networks that are 10$\times$ larger than the ones supported by existing analysis techniques. We believe that our approach to estimating tight output bounds of a network for a given input range can also help improve the explainability of neural networks and guide the training process of more robust neural networks.

==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

Our implemented \sys in about 26,000 lines of \texttt{C} code. In our initial experiments we found out that the performance of matrix multiplications is a major determining factor for the overall performance of the symbolic relaxation and interval propagation process. We use the highly optimized \texttt{OpenBLAS}\footnote{https://www.openblas.net/} library for matrix multiplication. We use {lp\_solve 5.5}\footnote{http://lpsolve.sourceforge.net/5.5/} for solving the linear constraints generated during the directed constraint refinement process. As formally checking non-existence of adversarial images that can be generated by a L-2 norm bounded attacker require us to solve an optimization problem where the constraints are linear but the objective is quadratic, we use the {Gurobi 8.0.0} solver as lp\_solve does not support quadratic objectives yet. All our evaluations were performed on a Linux server running Ubuntu 16.04 with 8 CPU cores and 256GB memory.

\noindent\textbf{\textit{Parallelization.}} Our directed constraint refinement process is highly parallelizable as it creates an independent set of linear programs that can be solved in parallel. For facilitating this process, \sys creates a thread pool where each thread solves one set of linear constraints with its own lp\_solve instances. However, as the refinement process might be highly uneven for different overestimated nodes, we periodically rebalance the queues of different threads to minimize idle CPU time.

\noindent\textbf{\textit{Outward Rounding.}} One of the side effects of floating point computations performed in DNNs is that even minor precision drops during analysis of one node and can be amplified significantly during through propagation through other layers. To avoid such issues, we perform outward rounding after every floating point computation, i.e., we always round $[\underline{x},\overline{x}]$ to $[\lfloor\underline{x}\rfloor, \lceil\overline{x}\rceil ]$. Our current prototype uses 32-bit \texttt{float} arithmetic that can support all of our current safety properties. However, if needed, the analysis can easily be switched to 64-bit \texttt{double}.

\noindent\textit{\textbf{Supporting Convolutional Layers.}} DNN with convolutional layers are often used in computer vision applications. Convolutional layers usually perform matrix multplication of some input values with a convolution kernal to get each output value as shown in  Figure~\ref{fig:convolution}. To propagate symbolic intervals through the convolutional layers, we simply multiply the symolic interval inputs with the concrete kernel to get the output symbolic intervals as shown in Figure~\ref{fig:convolution}.  


\begin{figure}[!hbt]
	\centering
	\includegraphics[width=\columnwidth]{image/conv_sym.pdf}
	\caption{Element-wise matrix multiplication of concrete inputs and a convolution kernel as performed in a DNN convolutional layer(upper). (Lower) propagating symbolic intervals through convolutional layers.}
	\label{fig:convolution}
\end{figure}


==> overview.tex <==
\section{Overview}
\label{sec:overview}

\begin{figure*}[!htb]
	\includegraphics[width=\textwidth]{image/DNNVerif1.pdf}
	\caption{Showing (a) symbolic linear relaxation results in tighter output range $[3.2,9]$ but still violated the safety property $f>3.3$. (b) further using one step of directed constraint refinement to split on overestimated node A and get refined output range $[3.5,9]$, formally proved save by linear solver.}
	\label{fig:interval_optimize}
\end{figure*}

In this section, we motivate the introduction of our two new methods, \textit{Symbolic Linear Relaxation} and \textit{Directed Constraint Refinement} through the same example in Section \ref{sec:background}. Here we define the safety property as $f>3.3$ that none of techniques described in Section \ref{sec:background} can prove.

\noindent\textbf{Symbolic Interval Relaxation.} Upon symbolic interval analysis \cite{reluval2018}, we keep the same symbolic intervals for node B and C in that their equations before ReLU are always positive. However, for node A, instead of directly applying a concretization, ignoring all the dependencies, we use tight linear lower and upper bound equations to relax the true output ranges in terms of input variables. As shown in Figure \ref{fig:interval_optimize}(a), we relax the node A output $Relu(2x-3y)$ to $[0.2(2x-3y),0.2(2x-3y+4)]$ instead of $[0,1]$ after concretization, leading to tighter output range $f=[3.2,9]$. It can provide great improvement over naive interval propagation and symbolic interval analysis because dependencies are partially kept.

\noindent\textbf{Directed Constraint Refinement.} Due to symbolic linear relaxation, we know that only node A has overestimation error. We define such special ReLU nodes like A as \texttt{overestimated node}. Based on them, directed constraint refinement iteratively splits them by combining directed constraints and reunion the results with the help of linear solver to refine the formal proof problem. Consider example shown in Figure \ref{fig:interval_optimize}(b), node A $ReLU(2x-3y)$ is marked as targeted overestimated node. We split original formal proof problem into two independent cases: (1) A is negative $2x-3y\leq0$, and (2) A is positive $2x-3y>0$. For these two cases, linear solver can tell respectively that neither of them violates the safety property $f>3.3$. Therefore, the property is successfully proved safe. Specifically, we can see the reunion of these two outputs is $[3.5,9]$ which is the tightest bound we can get.


==> related.tex <==
\section{Related Work}
\label{sec:related}

Formal analysis systems of neural network start from extending existing solvers used in traditional programming verifiers. One of the earliest ones was Hysat, which, while groundbreaking, could only efficiently run on networks with on the order of 20 hidden nodes \cite{pulina2010abstraction}. Another one of this type, found in \cite{huang2017safety}, uses the z3 solver to do a brute force check of all possible manipulations for an image. Likewise, \cite{ehlers2017formal} leveraged their Planet solver to handle piecewise linear NN. While these works were major milestones, they have been outclassed by more state-of-the-art systems, such as Reluplex \cite{katz2017reluplex, katz2017towards}. It could handle larger networks by expanding the theory around the simplex algorithm to handle Relu node relationships. Nonetheless, Reluplex is still inefficient so that it did not scale well to larger networks more than 1,000 intermediate nodes. There has additionally been work done by \cite{peck2017lower,weng2018evaluating}, who look for lower bounds of perturbations given output ranges via estimating a network's Lipschitz constant or layer architecture, but the theoretical bound they give contains large false positive.

Currently, formal analysis systems tend to get rid of solvers. VeriVis from \cite{pei2017towards}, for example, is a black-box system that does a brute-force check of all possible perturbations in a small specified input range. PixelDP from~\cite{pixeldp} leverages differential privacy to provide certain robustness guarantee but with small norm bounded range. In contrast, the majority of non-solver-based methods leverage classic abstract domains and achieve good results. \cite{kolter2017provable} and its similar work \cite{raghunathan2018certified}, though proposed for robust training, leverage polytope and its duality problem to give a useful upper bound of adversarial cases. $AI^2$~\cite{gehrai} utilizes zonotope to give a tighter approximated output ranges for non-box input space. They can provide some guarantee for larger networks, but the drawback is they are all one-shot output range approximations and can do nothing when the adversarial property is still not formally proved. More recently, ReluVal~\cite{reluval2018} has been proposed, which leverages symbolic interval propagation and iterative input refinement, and therefore is able to prove the same properties as Reluplex on ACAS Xu around 200 times more efficiently. However, their performance is hindered by naive interval propagation, and also they cannot scale to handle networks with many input nodes. \textbf{Robust training leverages such relaxation methods and train robust networks.}

Unlike previous work, the proposed symbolic linear relaxation and directed constraint refinement in \sys offers an improvement from an efficiency standpoint over the aforementioned solvers. \sys can efficiently provide a tight output bound and thus can be used to greatly improve the performance of~\cite{ehlers2017formal,reluval2018}. Furthermore, the splitting involved in directed constraint refinement of overestimated nodes allows for parallelization and has potential to increase the performance of robust training process like~\cite{kolter2017provable,raghunathan2018certified}.

\begin{comment}
\noindent\textbf{\textit{Formal verification of DNNs.}} Formal DNN verifiers start from extending existing solvers used in traditional programming verification systems. One of the earliest ones was Hysat, which, while groundbreaking, could only efficiently run on networks with on the order of 20 hidden nodes \cite{pulina2010abstraction}. Another example of this type, found in \cite{huang2017safety}, uses the z3 solver to do a brute force check of all possible manipulations for an image in a specified range. Likewise,\cite{ehlers2017formal} leveraged their Planet solver to handle piecewise linear NN. While these works were major milestones, they have been outclassed by more state-of-the-art verifiers, such as Reluplex \cite{katz2017reluplex, katz2017towards}. Reluplex, could handle larger networks by expanding the theory around the simplex algorithm to handle Relu node relationships. It has even been used by \cite{carlini2017towards} to find ground-truth adversarial examples nearest to a test input. Nonetheless, this verifier was still inefficient, and moreover non-parallelizable, so it did not scale well to even larger networks, struggling to perform on networks containing more than 1,000 intermediate nodes. There has additionally been work done by \cite{peck2017lower,weng2018evaluating}, who look for lower bounds of perturbations given output ranges via estimating a network's Lipschitz constant or layer architecture.

Currently verifiers tend to get rid of solver. VeriVis from \cite{pei2017towards}, for example, is a black-box system that does a brute-force check of all possible perturbations in a small specified input range. But majority of non-solver-based verification systems, leveraging classic abstract domains, are proposed and achieve good results, \cite{kolter2017provable} and its similar work\cite{raghunathan2018certified}, though proposed for robust training, leverage polytope and its duality problem to give a useful upper bound of adversarial cases. $AI^2$\cite{gehrai} utilizes zonotope to give a tighter approximated output ranges for non-box input space. They can provide some guarantee for larger networks, but the drawback is they are all one-shot output range approximations and can do nothing when the adversarial property is still not verified. More recently, \cite{reluval2018} has been proposed, which leverages, much like in \sys, symbolic interval propagation and iterative input refinement, and therefore is able to prove the same properties as Reluplex on ACAS Xu around 200 times more efficiently. However, their performance is hindered by naive interval propagation, and also they cannot scale to handle networks with many input nodes.

The proposed symbolic linear relaxation and directed constraint refinement of overestimated nodes in \sys offers an improvement from an efficiency standpoint over the aforementioned solvers. \sys can efficiently provide a tight output bound and thus can be used to greatly improve the performance of\cite{ehlers2017formal,reluval2018}. Furthermore, the splitting involved in directed constraint refinement of overestimated nodes allows for parallelization while refining the search space, which is a property that \cite{katz2017reluplex} could not leverage.


\noindent\textbf{Adversarial examples and attacks.} Adversarial examples, a phenomenon first noticed in \cite{szegedy2013intriguing}, are minor perturbations of inputs that lead a NN to misclassification. An early attack to leverage adversarial examples was FGSM, which was proposed by \cite{goodfellow2014explaining}. Following this early construction, many other attacks were developed using either gradient-based or black-box methods. Examples of these approaches include JSMA\cite{papernot2016limitations}, CW\cite{carlini2017towards}, BIM\cite{kurakin2016adversarial}, DeepFool\cite{moosavi2016deepfool}, and many others\cite{papernot2016practical, liu2016delving, nguyen2015deep, xu2016automatically}. Today, almost all of the aforementioned attacks are collected in the \texttt{Cleverhans} library \cite{papernot2016cleverhans}. However, due to the fact that almost all neural networks are not convex, the procedures cannot find global extrema, and thus cannot guarantee non-existence of adversarial examples. \sys, in contrast, guided by our model of symbolic linear relaxation and direct constraint refinement on overestimated nodes, not only can provide formal guarantees on large-scale networks, but is also has a stronger ability to narrow down adversarial ranges and locate adversarial examples.

\noindent\textbf{Testing and Defense Systems.} Many testing and defense systems have been proposed as a result of the increasing awareness and prevalence of adverarial examples in DNN. Much of previous work has focused on improving the robustness and reliability of DNNs, including the works \cite{carlini2017towards, cisse2017parseval, gu2014towards, papernot2017extending,papernot2016distillation,goodfellow2014explaining, zheng2016improving}. However, while these systems do offer improved defense, they are still susceptible under stronger attack systems, such as those by \cite{carlini2017towards,carlini2016defensive,tramer2017ensemble}. To lessen the requirement of manual input into testers, DeepXplore\cite{pei2017deepxplore} was proposed to systematically test large-scale networks through gradient-based differential testing.Currently, leveraging polytope and duality, \cite{kolter2017provable, raghunathan2018certified} provide robust training that can create network robust against adversarial. However, their robust training takes much more time and lower prediction accuracy compared to normal training. \sys, though is a verification system, has the potential to be perfectly fit into robust training and achieve better performance, which is something we leave for future work.

\end{comment}







